AttackLLM: LLM-based Attack Pattern Generation for an Industrial Control System

Malicious examples are crucial for evaluating the robustness of machine learning algorithms under attack, particularly in Industrial Control Systems (ICS). However, collecting normal and attack data in ICS environments is challenging due to the scarcity of testbeds and the high cost of human expertise. Existing datasets are often limited by the domain expertise of practitioners, making the process costly and inefficient. The lack of comprehensive attack pattern data poses a significant problem for developing robust anomaly detection methods. In this paper, we propose a novel approach that combines data-centric and design-centric methodologies to generate attack patterns using large language models (LLMs). Our results demonstrate that the attack patterns generated by LLMs not only surpass the quality and quantity of those created by human experts but also offer a scalable solution that does not rely on expensive testbeds or pre-existing attack examples. This multi-agent based approach presents a promising avenue for enhancing the security and resilience of ICS environments.

==> Prompts.tex <==

\begin{markdown}


### Prompt for LLM:

**Context:**
The provided dataset is from a water treatment plant called SWaT (Secure Water Treatment), which is composed of six stages. This dataset represents **Stage 1** of the process under normal operation. The dataset includes the following sensors and actuators:

- **Sensors:**
  - `FIT101`: Flow rate measurement.
  - `LIT101`: Level measurement.

- **Actuators:**
  - `MV101`: Motorized valve (2 = open, 1 = closed, 0 = moving).
  - `P101`: Pump 1 (2 = on, 1 = off).
  - `P102`: Pump 2 (2 = on, 1 = off).

The dataset contains time-series data with timestamps, sensor readings, and actuator states.

---

**Tasks:**

1. **Learn the Control Logic:**
   - Analyze the provided time-series data to infer the control logic governing the interaction between the sensors (`FIT101`, `LIT101`) and actuators (`MV101`, `P101`, `P102`).
   - Identify patterns or rules that describe how the actuators respond to changes in sensor readings.
   - For example:
     - Under what conditions does `MV101` open or close?
     - How do `P101` and `P102` respond to changes in `LIT101` or `FIT101`?

2. **Generate Control Invariants:**
   - Based on the inferred control logic, generate **control invariants** that describe the expected behavior of the system under normal operation.
   - Control invariants are properties or conditions that must always hold true for the system to operate correctly. For example:
     - If `LIT101` exceeds a certain threshold, `MV101` should close.
     - If `FIT101` drops below a certain value, `P101` should turn on.

3. **Provide Structured Text for PLC Programming:**
   - Translate the inferred control logic into **structured text** that can be programmed into a Programmable Logic Controller (PLC).
   - Use a format that is clear and compatible with PLC programming languages (e.g., ladder logic, structured text, or function block diagrams).
   - For example:
     - If `LIT101 > 120`, then `MV101 = 0` (close the valve).
     - If `FIT101 < 10`, then `P101 = 1` (turn on Pump 1).

---

**Output Format:**

1. **Control Logic Summary:**
   - Provide a concise summary of the inferred control logic, including the conditions under which each actuator operates.

2. **Control Invariants:**
   - List the control invariants derived from the data.

3. **Structured Text for PLC:**
   - Provide the control logic in a structured text format suitable for PLC programming.


**Additional Notes:**
- If the dataset does not provide sufficient information to infer certain control rules, please indicate this and suggest additional data or experiments that might be needed.
- Ensure that the generated control logic and invariants are consistent with the provided data and reflect the normal operation of the system.

---

### Follow-up query

Can you provide the mentioned thresholds based on the data from the provided time series? Also, all possible invariants are stated as a combination of all sensors and actuators. surely these could be learned from the time series data.

### Design document
Let me provide the control strategy for stage 1 from the design document and see how that change your outputs:Control Strategy For stage1
1) Raw water inlet valve (MV-101) shall be activated by raw water tank level (LIT-
101)
a. Low Setpoint: 500mm -->  Valve MV-101 OPEN
b. High Setpoint: 800mm --> Valve MV-101 CLOSE
c. Low Low Setpoint: 250mm --> Alarm & Pump P-101/ P-102 STOP
d. High High Setpoint: 1200mm --> Alarm
2) Raw water pump (P-101 & P-102) shall be interlocked with
a. One duty, one standby
b. To interlocked with UF feedwater tank level (LIT-201)
i. Low Setpoint: 800mm --> Pump P-101/ P-102 START
ii. High Setpoint: 1000mm --> Pump P-101/ P-102 STOP
c. To interlocked with Feedwater flowmeter (FIT-201)
i. Low Setpoint: 0.5m3/h --> Pump P-101/ P-102 STOP

### Validation Query

can you validate  the control from the design corresponds to one reflected from the time series data?



\end{markdown}

